MCPMark: A Benchmark for Stress-Testing Realistic and Comprehensive MCP Use

MCP standardizes how LLMs interact with external systems, forming the foundation for general agents. However, existing MCP benchmarks remain narrow in scope: they focus on read-heavy tasks or tasks with limited interaction depth, and fail to capture the complexity and realism of real-world workflows. To address this gap, we propose MCPMark, a benchmark designed to evaluate MCP use in a more realistic and comprehensive manner. It consists of $127$ high-quality tasks collaboratively created by domain experts and AI agents. Each task begins with a curated initial state and includes a programmatic script for automatic verification. These tasks demand richer and more diverse interactions with the environment, involving a broad range of create, read, update, and delete (CRUD) operations. We conduct a comprehensive evaluation of cutting-edge LLMs using a minimal agent framework that operates in a tool-calling loop. Empirical results show that the best-performing model, gpt-5-medium, reaches only $52.56$\% pass@1 and $33.86$\% pass^4, while other widely regarded strong models, including claude-sonnet-4 and o3, fall below $30$\% pass@1 and $15$\% pass^4. On average, LLMs require $16.2$ execution turns and $17.4$ tool calls per task, significantly surpassing those in previous MCP benchmarks and highlighting the stress-testing nature of MCPMark.

==> tables/benchmark_stat.tex <==
\begin{wraptable}{r}{0.45\textwidth}
\centering
\caption{Average and maximum statistics of \texttt{MCPMark} tasks, and counts of tasks and initial states per MCP environment.}
{\small
\begin{tabular}{l r r r}
\toprule
 & Mean & Max &  \\
\midrule
\# Words & 288.6 & 5342 & \\
\# Lines & 209.8 & 641  & \\
\midrule
MCP & \# Tasks & \# Initial States & \\
\midrule
Filesystem  & 30 & 10 & \\
GitHub      & 23 &  6 & \\
Notion      & 28 & 10 & \\
Playwright  & 25 &  5 & \\
PostgreSQL  & 21 &  7 & \\
\bottomrule
\end{tabular}
}
\vspace{-2.5em}
\end{wraptable}
